Are 140 Characters Enough? A Large-Scale Linkability Study of Tweets

Microblogging is a very popular Internet activity that informs and entertains great multitudes of people world-wide via quickly and scalably disseminated terse messages containing all kinds of newsworthy utterances. Even though microblogging is neither designed nor meant to emphasize privacy, numerous contributors hide behind pseudonyms and compartmentalize their different incarnations via multiple accounts within the same, or across multiple, site(s). Prior work has shown that stylometric analysis is a very powerful tool capable of linking product or service reviews and blogs that are produced by the same author when the number of authors is large. In this paper, we explore linkability of tweets. Our results, based on a very large corpus of tweets, clearly demonstrate that, at least for relatively active tweeters, linkability of tweets by the same author is easily attained even when the number of tweeters is large. We also show that our linkability results hold for a set of actual Twitter users who tweet from multiple accounts. This has some obvious privacy implications, both positive and negative.

==> conclusion.tex <==
\section{Conclusion}
\label{conclusion}
%
\if 0 
In this paper, we reported on a large-scale linkabilty analysis of tweets. 
We based our study on two datasets, each consisting of more than $8,000$ tweeters. We showed 
that tweets in all datasets are highly linkable, even when we only rely 
on unigram and bigram distributions. We re-produced our linkability analysis on a set of 14 dual-accounts that belong to the same owners and the linkability results were comparably high. Our linkability analysis 
results should be very troubling for tweeters who are concerned about 
their privacy. 
\fi 
This paper reported on a large-scale linkability analysis of tweets.
It was based on two datasets, each consisting of over $8,000$ tweeters.
We showed that tweets are highly linkable, even when we only rely
on unigram and/or bigram distributions. We also performed linkability analysis
over a small set of actual dual-account users and linkability remained quite high.

